Tester versus Bug: A Generic Framework for Model-Based Testing via Games

We propose a generic game-based approach for test case generation. We set up a game between the tester and the System Under Test, in such a way that test cases correspond to game strategies, and the conformance relation ioco corresponds to alternating refinement. We show that different test assumptions from the literature can be easily incorporated, by slightly varying the moves in the games and their outcomes. In this way, our framework allows a wide plethora of game-theoretic techniques to be deployed for model based testing.

==> eptcsdata.tex <==
\providecommand{\firstpage}{118}
\providecommand{\publicationstatus}{A. Orlandini, M. Zimmermann (Eds.): 9th Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF'18)\\
EPTCS 277, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.277.9}{10.4204/EPTCS.277.9}}

